Retro-Actions: Learning 'Close' by Time-Reversing 'Open' Videos

We investigate video transforms that result in class-homogeneous label-transforms. These are video transforms that consistently maintain or modify the labels of all videos in each class. We propose a general approach to discover invariant classes, whose transformed examples maintain their label; pairs of equivariant classes, whose transformed examples exchange their labels; and novel-generating classes, whose transformed examples belong to a new class outside the dataset. Label transforms offer additional supervision previously unexplored in video recognition benefiting data augmentation and enabling zero-shot learning opportunities by learning a class from transformed videos of its counterpart. Amongst such video transforms, we study horizontal-flipping, time-reversal, and their composition. We highlight errors in naively using horizontal-flipping as a form of data augmentation in video. Next, we validate the realism of time-reversed videos through a human perception study where people exhibit equal preference for forward and time-reversed videos. Finally, we test our approach on two datasets, Jester and Something-Something, evaluating the three video transforms for zero-shot learning and data augmentation. Our results show that gestures such as zooming in can be learnt from zooming out in a zero-shot setting, as well as more complex actions with state transitions such as digging something out of something from burying something in something.

==> Makefile <==
# You want latexmk to *always* run, because make does not have all the info.
# Also, include non-file targets in .PHONY so they are run regardless of any
# file of the given name existing.
DOC_SRC:=$(shell find . -maxdepth 1 -iregex './[^.].*\.tex')
MEDIA_SRC:=$(shell find images -type f)
SVG_SRC := $(shell find images -type f -iname '*.svg')
PDF_SVG := $(patsubst %.svg,%.pdf,$(SVG_SRC))
DEPS := $(DOC_SRC) $(MEDIA_SRC) $(PDF_SVG) $(BIB_FILES)
BIB_FILES:= ~/references.bib
.PHONY: all clean
.SECONDARY: $(PDF_SVG)

all: video-reversal.pdf

# -pdf tells latexmk to generate PDF directly (instead of DVI).
# -pdflatex="" tells latexmk to call a specific backend with specific options.
# -use-make tells latexmk to call make for generating missing files.
# -interaction=nonstopmode keeps the pdflatex backend from stopping at a
#     missing file reference and interactively asking you for an alternative.

%.pdf: %.tex $(DEPS)
	latexmk -f -pdf -pdflatex="pdflatex -interaction=nonstopmode --shell-escape" -use-make $<

%.pdf: %.svg
# Inkscape v0.9X
#	inkscape $< --export-area-drawing --without-gui --export-type=pdf --export-file $@
# Inkscape v1.0+
	inkscape $< --export-area-drawing --without-gui --export-pdf $@

clean:
	latexmk -C $(DOC_SRC)

